QTRAN++: Improved Value Transformation for Cooperative Multi-Agent Reinforcement Learning

QTRAN is a multi-agent reinforcement learning (MARL) algorithm capable of learning the largest class of joint-action value functions up to date. However, despite its strong theoretical guarantee, it has shown poor empirical performance in complex environments, such as Starcraft Multi-Agent Challenge (SMAC). In this paper, we identify the performance bottleneck of QTRAN and propose a substantially improved version, coined QTRAN++. Our gains come from (i) stabilizing the training objective of QTRAN, (ii) removing the strict role separation between the action-value estimators of QTRAN, and (iii) introducing a multi-head mixing network for value transformation. Through extensive evaluation, we confirm that our diagnosis is correct, and QTRAN++ successfully bridges the gap between empirical performance and theoretical guarantee. In particular, QTRAN++ newly achieves state-of-the-art performance in the SMAC environment. The code will be released.

==> 4.1.algo_QOPT.tex <==
\begin{algorithm}[t]
\caption{\algname}
 \label{algo:QOPT}
 \begin{spacing}{1.1}
 \begin{algorithmic}[1]
 \STATE Initialize replay memory $\mathcal{B}\leftarrow \emptyset$ and target parameters $\theta^- \gets \theta$
 \FOR{episode = 1 to $M$}
 \STATE Observe initial state $\bm{s}^0$ and observation $\bm{o}^0 = [O(\bm{s}^0,i)]_{i=1}^N$ for each agent $i$
    \FOR{$t = 1$ to $T$}
        \STATE With probability $\epsilon$, select an action $u^t_i$
        \STATE Otherwise, set $u^t_i = \arg\max_{u^t_{i}}q_i(\tau^t_i,u^t_i)$ for each agent $i$
        \STATE Take action $\bm{u}^t$, and retrieve next state and reward $(s^{t+1},r^t)$
        \STATE Store transition $(s^t, \bm{u}^t, r^t, s^{t+1})$ in $\mathcal{B}$
        \STATE Sample a transition $(s, \bm{u}, r, s')$ from $\mathcal{B}$
         %\STATE Let $y^{\text{dqn}}(r, s'; \bm{\theta^{-}}) = r + \gamma\Qtot(s', \bm{\bar{u}}';\bm{\theta} ^{-})$ and $ \bar{\bm{u}}' = [\arg\max_{u_{i}}q_i(\tau'_i,u_i;\bm{\theta}^{-})]_{i=1}^N$
        \STATE Update $\theta$ by minimizing the losses $L_{td}$ and $L_{opt}$ from Equation~\eqref{eq:td_loss} and \eqref{eq:opt_loss0}, respectively:
        \begin{equation*}
        L(s, \bm{u}, r, s'; \bm{\theta}) = L_{td}(s, \bm{u}, r, s'; \bm{\theta}) + \lambda_{opt} L_{\text{opt}}(s, \bm{u}, r, s'; \bm{\theta})
        \end{equation*}
        \STATE Update target network parameters $\theta^- \gets \theta$ with period $I$
 \ENDFOR
 \ENDFOR
 \end{algorithmic}
 \end{spacing}
  \end{algorithm}

 %  ,\cr
% L_{\text{td}}(s, \bm{u}, r, s';\bm{\theta}) &= \big(\Qtot(s,\bm{u}) - y^{\text{dqn}}(r, s'; \bm{\theta}^{-})\big)^{2}.
        %\begin{subequations}
%  \begin{align*}[left ={L_{\text{opt}}(s, \bm{u}, r, s';\bm{\theta}) = \empheqlbrace}]
%    & (\Qtot(s,\bm{u}) - \Qtot'(s,\bm{u}))^2         &\Qtot(s,\bm{u}) > \Qtot(s,\bm{\bar{u}}),  \\
%    & (clip(\Qtot'(s,\bm{u}), \Qtot(s,\bm{\bar{u}}), \Qtot(s,\bm{u}))- \Qtot'(s,\bm{u}))^2  &\Qtot(s,\bm{u}) < \Qtot(s,\bm{\bar{u}}),
%  \end{align*}
%  \end{subequations}
% \begin{align*}
%     L_{\text{opt}}(s, \bm{u}, r, s';\bm{\theta}) = 
%     \begin{cases}
%     (\Qtot(s,\bm{u}) - \Qtot'(s,\bm{u}))^2,         &\Qtot(s,\bm{u}) > \Qtot(s,\bm{\bar{u}}), \\
%     (\mathtt{clip}(\Qtot'(s,\bm{u}), \Qtot(s,\bm{\bar{u}}), \Qtot(s,\bm{u}))- \Qtot'(s,\bm{u}))^2,  &\Qtot(s,\bm{u}) < \Qtot(s,\bm{\bar{u}}),
%     \end{cases}
% \end{align*}  
        %\STATE $s = s^{\text{temp}}$


==> 4.2.matrixgame.tex <==
\begin{table}[t]
% \scriptsize
\setlength{\tabcolsep}{-1pt}
        \caption{Payoff matrix of the one-step non-decentralizable game and reconstructed results of the game. States $s_{1}$ and $s_{2}$ are randomly selected with same probability and the agents cannot observe the state. Boldface means optimal and greedy actions from the state-action value function.}
    \begin{minipage}{.48\columnwidth}
      \centering
      \begin{minipage}{.48\columnwidth}
      \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{4}& 2 \\ \hline
        B & 2 & 0 \\ \hline
        \end{tabular}
        \end{minipage}
        \begin{minipage}{.48\columnwidth}
        \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & 0& 1 \\ \hline
        B & 1 & \textbf{2} \\ \hline
        \end{tabular}
        \end{minipage}
        \subcaption{Payoff of matrix game for state $s_1$ and $s_2$}
        \label{table:p1-appendix}
    \end{minipage}
    \begin{minipage}{.48\columnwidth}
      \centering
      \begin{minipage}{.48\columnwidth}
      \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{2.0}& 1.5 \\ \hline
        B & 1.5 & 1.0 \\ \hline
        \end{tabular}
        \end{minipage}
        \begin{minipage}{.48\columnwidth}
        \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{2.0}& 1.5 \\ \hline
        B & 1.5 & 1.0 \\ \hline
        \end{tabular}
        \end{minipage}
        \subcaption{VDN: $\Qtot$}
        \label{table:p2-appendix}
    \end{minipage} \\
    \begin{minipage}{.48\columnwidth}
      \centering
      \begin{minipage}{.48\columnwidth}
      \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{4.0}& 2.0 \\ \hline
        B & 2.0 & 0.0 \\ \hline
        \end{tabular}
        \end{minipage}
        \begin{minipage}{.48\columnwidth}
        \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{1.0}& 1.0 \\ \hline
        B & 1.0 & 1.0 \\ \hline
        \end{tabular}
        \end{minipage}
        \subcaption{QMIX case 1: $\Qtot(s_1), \Qtot(s_2)$}
        \label{table:p3-appendix}
    \end{minipage}
    \begin{minipage}{.48\columnwidth}
      \centering
      \begin{minipage}{.48\columnwidth}
      \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & 3.0& \textbf{3.0} \\ \hline
        B & 1.0 & 1.0 \\ \hline
        \end{tabular}
        \end{minipage}
        \begin{minipage}{.48\columnwidth}
        \centering\end{table}

        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & 0.5& \textbf{1.5} \\ \hline
        B & 0.5 & 1.5 \\ \hline
        \end{tabular}
        \end{minipage}
        \subcaption{QMIX case 2: $\Qtot(s_1), \Qtot(s_2)$}
        \label{table:p4-appendix}
    \end{minipage} \\
    \begin{minipage}{.48\columnwidth}
      \centering
      \begin{minipage}{.48\columnwidth}
      \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{3.0}& 2.0 \\ \hline
        B & 2.5 & 1.5 \\ \hline
        \end{tabular}
        \end{minipage}
        \begin{minipage}{.48\columnwidth}
        \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{1.0}& 1.0 \\ \hline
        B & 0.5 & 0.5 \\ \hline
        \end{tabular}
        \end{minipage}
        \subcaption{$\algname$ head 1: $\Qtran^{(1)}(s_1), \Qtran^{(1)}(s_2)$}
        \label{table:p5-appendix}
    \end{minipage}
    \begin{minipage}{.48\columnwidth}
      \centering
      \begin{minipage}{.48\columnwidth}
      \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{3.0}& 2.5 \\ \hline
        B & 2.0 & 1.5 \\ \hline
        \end{tabular}
        \end{minipage}
        \begin{minipage}{.48\columnwidth}
        \centering
        \begin{tabular}{|P{1.0cm}||P{1.0cm}|P{1.0cm}|}
        \hline
        & A & B\\ \hline \hline
        A & \textbf{1.0}& 0.5 \\ \hline
        B & 1.0 & 0.5 \\ \hline
        \end{tabular}
        \end{minipage}
        \subcaption{$\algname$ head 2: $\Qtran^{(2)}(s_1), \Qtran^{(2)}(s_2)$}
        \label{table:p6-appendix}
    \end{minipage}
\vspace{-0.2cm}
\label{table:matrix-appendix}
\end{table}

==> 4.method_old.tex <==

% Move "Training" to the left
% Change the subscripts of L
% Modularize Qtran and Qtran-adv, and note that they do not run simultaneously
% Do something about the empty spaces on either side

% \begin{figure*}[!t]
%   \centering
%  \includegraphics[width=0.92\textwidth]{figure/NN_QREG.pdf}
% \caption{$\algoname$ Architecture}
%   \label{fig:qreg}
% \end{figure*}

% \begin{figure*}[h]
%   \centering
%  \includegraphics[width=0.92\textwidth]{figure/NN_QREG-adv.pdf}
% \caption{$\algoname$-adv Architecture}
%   \label{fig:qreg-adv}
% \end{figure*}





\section{QOPT}

\subsection{Problem formulation}

In our work, we take decentralized partially observable Markov Decision Process (Dec-POMDP) \cite{oliehoek2016concise} to model fully cooperative multi-agent tasks consisting of a tuple $\set{G} = <\set{S},\set{U},P,r,\set{Z},O,N,\gamma>$. First, $\bm{s} \in \set{S}$ is the true state of the environment. At each time step, each agent $i \in \set{N} := \{1,...,N\}$ selects an action $u_i \in \set{U}$ and joint action vector, $\bm{u} := [u_i]_{i=1}^N \in \set{U}^N$. It causes a stochastic transition of environment, and $P(\bm{s}'|\bm{s},\bm{u}):\set{S}\times \set{U}^N \times \set{S} \mapsto [0,1]$ describes the state transition dynamics. All agent share the same reward $r(\bm{s},\bm{u}):\set{S} \times \set{U}^N \mapsto \real $, and $\gamma \in [0,1)$ is the discount factor. Each agent has an individual partial observation according to their own observation function $O(\bm{s},i) : \set{S} \times \set{N} \mapsto \set{Z}$ and action-observation history $\tau_i \in \set{T} := (\set{Z} \times \set{U})^{*}.$

\subsection{Method}

\begin{figure*}[!t]
  \centering
 \includegraphics[width=0.93\textwidth]{figure/QOPT.pdf}
\caption{QOPT Architecture \textcolor{red}{Temporal}}
  \label{fig:qreg}
\end{figure*}

In this part, we propose a new method, which we call QOPT. The primary objective of our design is to obtain a decentralizable architecture. Figure~\ref{fig:qreg} shows the overall neural network architecture of our algorithm. For each agent, DRQN \cite{hausknecht2015deep} represent individual action-value networks. At each time step, agents receive hidden states and their local observations as inputs and calculate their individual action-value. 

Mixing networks are a feed-forward network that takes individual action-values $Q_i$ as inputs and outputs joint action-value $\Qtot$ and optimistic joint action-value $\Qtot'$. For the optimistic joint action value, monotonicity constraints is satisfied by restricting all weights in the mixing network to be non-negative values. The non-negative weights of mixing network naturally hold the monotonicity and ensure that optimal actions of the joint action-value function are the same as the optimal ones of the individual action-value functions. Since the joint action-value function does not have the monotonic restriction, more complex action-value can be estimated by joint action-value function but the natural decomposition property disappears.

The weights in the mixing network are the output of hypernetworks \cite{ha2017hypernetworks} to condition the weights on the state, which is available only during training. The hypernetworks receive state information as input and generates the conditioned weights for mixing networks, and it makes integrating the full state information into the joint action-value estimation. By an absolute activation function, hypernetworks ensure that the mixing weights of optimistic joint action-value function are non-negative. The detailed architectures for networks are the same as in QMIX \cite{pmlr-v80-rashid18a} and SMAC \cite{samvelyan19smac}.



\subsection{Loss functions}

In the QOPT, there are two goals in centralized training. One is to train the joint action-value function for estimating true action-value and the other is an optimistic action-value function so that optimal actions of the optimistic and original action-value function should be equal. To train joint action-value function $\Qtot$ with non-monotonic mixing network, we use the DQN \citep{mnih2015human} loss with target network and replay buffer which store the sample $(\vec{\tau},\vec{u},r, \vec{\tau}')$. We update the network parameters to minimize the loss function defined as 


\begin{align*}
L_{\text{td}}(;\bm{\theta})&= \big(\Qtot(\bm{\tau},\bm{u}) - y^{\text{dqn}}(r, \bm{\tau}'; \bm{\theta}^{-})\big)^{2},\cr 
\end{align*} 
where 
$y^{\text{dqn}}(r, \bm{\tau}'; \bm{\theta^{-}}) = r + \gamma
\Qtot(\bm{\tau}', \bm{\bar{u}}';\bm{\theta} ^{-}),$ $ \bar{\bm{u}}' = [\arg\max_{u_{i}}Q_i(\tau'_i,u_i;\bm{\theta}^{-})]_{i=1}^N,$ and $\bm{\theta}^{-}$ are target network parameters from $\bm{\theta}$, as in DQN \citep{mnih2015human}. 

We introduce additional loss function to learn the optimistic joint action-value function $\Qtot'$ with monotonic mixing network for policy decentralization.

% \begin{subnumcases}{\label{eq:regular_cond0}\hspace{-0.7cm}\sum_{i=1}^N Q_i(\tau_i,u_i) \! -\! \Qtot(\bm{\tau},\bm{u}) \! +\!\Vtot(\bm{\tau})\!=\!}
%     \!\!\! 0 & $\hspace{-0.5cm}\bm{u} = \bm{\bar{u}},$ \label{eq:regular_cond1}\\
%     \!\!\! \geq 0 & $\hspace{-0.5cm}\bm{u} \neq \bm{\bar{u},}$ \label{eq:regular_cond2}
% \end{subnumcases}

\begin{subnumcases}{{\label{eq:opt_loss0}}\hspace{-1.0cm}L_{\text{opt}}(;\bm{\theta})=}
    \!\!\! (\Qtot(\bm{\tau},\bm{u}) - \Qtot'(\bm{\tau},\bm{u}))^2 & $\hspace{0.0cm}\Qtot(\bm{\tau},\bm{u}) > \Qtot(\bm{\tau},\bm{\bar{u}}),$ {\label{eq:opt_loss1}}\\
    \!\!\! (clip(\Qtot'(\bm{\tau},\bm{u}), \Qtot(\bm{\tau},\bm{\bar{u}}), \Qtot(\bm{\tau},\bm{u}))- \Qtot'(\bm{\tau},\bm{u}))^2 & $\hspace{0.0cm}\Qtot(\bm{\tau},\bm{u}) < \Qtot(\bm{\tau},\bm{\bar{u}}),$ {\label{eq:opt_loss2}}
\end{subnumcases}
where $ \bar{\bm{u}} = [\arg\max_{u_{i}}Q_i(\tau_i,u_i;\bm{\theta}^{-})]_{i=1}^N.$

\vspace{0.5cm}

\begin{align}
    \Qtot'(\bm{\tau}, \bm{\bar{u}}) = \Qtot(\bm{\tau}, \bm{\bar{u}}) \label{eq:opt_cond0}\\
    \Qtot(\bm{\tau}, \bm{\bar{u}}) \geq \Qtot'(\bm{\tau},\bm{u}) \geq \Qtot(\bm{\tau}, \bm{u}) \label{eq:opt_cond1}
\end{align}

\vspace{0.5cm}

% \begin{subnumcases}{{\label{eq:opt_cond0}}\hspace{-1.0cm}\Qtot'(\bm{\tau},\bm{u}))=}
%     \!\!\! (\Qtot(\bm{\tau},\bm{u}) - \Qtot'(\bm{\tau},\bm{u}))^2 & $\hspace{0.0cm}\Qtot(\bm{\tau},\bm{u}) > \Qtot(\bm{\tau},\bm{\bar{u}}),$ {\label{eq:opt_loss1}}\\
%     \!\!\! (clip(\Qtot'(\bm{\tau},\bm{u}), \Qtot(\bm{\tau},\bm{\bar{u}}), \Qtot(\bm{\tau},\bm{u}))- \Qtot'(\bm{\tau},\bm{u}))^2 & $\hspace{0.0cm}\Qtot(\bm{\tau},\bm{u}) < \Qtot(\bm{\tau},\bm{\bar{u}}),$ {\label{eq:opt_loss2}}
% \end{subnumcases}
% where $ \bar{\bm{u}} = [\arg\max_{u_{i}}Q_i(\tau_i,u_i;\bm{\theta}^{-})]_{i=1}^N.$


\begin{theorem}
\label{thm:sufficiency}
A joint acton-value function $\Qtot(\bm{\tau}, \bm{u})$ is decentralized by $[Q_i(\tau_i, u_i)],$ if condition \eqref{eq:opt_cond1} holds

\end{theorem}

\begin{proof}
    Theorem~\ref{thm:sufficiency} shows that if conditions \eqref{eq:opt_cond0} hold, then $Q_i(\tau_i,u_i)$ satisfies optimal decentralization. We will show that   $\arg\max_{\bm{u}} \Qtot(\bm{\tau},\bm{u}) = \bm{\bar{u}}$. Recall
  that $\bar{u}_{i} = \arg\max_{u_{i}}Q_i(\tau_i,u_i)$ and
  $\bm{\bar{u}} = [\bar{u}_{i}]_{i=1}^N,$.
  
  \begin{align*}
\Qtot(\bm{\tau},\bm{\bar{u}}) &= \Qtot'(\bm{\tau}, \bm{\bar{u}}) \quad(\text{From} \; \eqref{eq:opt_cond0}) \\
&\geq \Qtot'(\bm{\tau}, \bm{{u}}) \quad(\text{From} \; \text{Monotonicity of }  \Qtot'(\bm{\tau}, \bm{{u}})) \\
&\geq \Qtot(\bm{\tau}, \bm{{u}}) \quad(\text{From} \; \eqref{eq:opt_cond0}).
\end{align*}
    It means that the set of local optimal actions $\bar{\bm u}$ maximizes
$\Qtot$, showing that $Q_i$ satisfies decentralizability.
\end{proof}

\begin{theorem}
\label{thm:necessity}
If there exists $\Qtot(\bm{\tau},\bm{u})$ and $[Q_i(\tau_i,u_i)]$ satisfying decentralizability, then there exists $\Qtot'(\bm{\tau}, \bm{u})$ that also satisfies conditions \eqref{eq:opt_cond0}. 
\end{theorem}

\begin{proof}
    By definition, if $\Qtot(\bm{\tau},\bm{u})$ is decentralized by $[Q_i(\tau_i,u_i)]$, then the following hold: (i)
  $\Qtot(\bm{\tau},\bar{\bm{u}}) -
  \max_{\bm{u}}\Qtot(\bm{\tau},\bm{u}) = 0$, (ii)
  $\Qtot(\bm{\tau},\bm{u}) - \Qtot(\bm{\tau},\bar{\bm{u}}) < 0$, and (iii) $\sum_{i=1}^N (Q_i(\tau_i,u_i) - Q_i(\tau_i,\bar{u}_i)) < 0$
\end{proof}

Conceptually, the optimistic joint action-value function follows the joint action-value function exactly only when the joint action-value is larger than threshold. Since small joint action-values are ignored, problems with limited representation complexity in QMIX alleviated and the optimistic joint action-value network allows tractable and efficient maximization.

Combining these two loss functions, we obtain the following objectives, which is minimized each iteration:

\begin{align}
  \label{eq:loss_total}
L(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta})=
 L_{\text{td}} + \lambda_\text{opt} L_\text{opt},
\end{align}
where $r$ is the reward for action $\bm{u}$ at observation histories $\bm{\tau}$ with transition to $\bm{\tau}'$. $\lambda_{\text{opt}}$ is the weight parameter to combine two loss functions in a weighted manner.

A sketch of the algorithm is presented in Algorithm~\ref{algo:QOPT}.

\begin{algorithm}[H]
 \caption{QOPT}
 \label{algo:QOPT}
 \begin{algorithmic}[1]
 \STATE Initialize replay memory $D$
 \STATE Initialize parameters $\theta$
 \STATE Initialize target parameters $\theta^- = \theta$
 \FOR{episode = 1 to $M$}
 \STATE Observe initial state $\bm{s}^0$ and observation $\bm{o}^0 = [O(\bm{s}^0,i)]_{i=1}^N$ for each agent $i$
    \FOR{$t = 1$ to $T$}
        \STATE With probability $\epsilon$ select a random action $u^t_i$
        \STATE Otherwise $u^t_i = \arg\max_{u^t_{i}}Q_i(\tau^t_i,u^t_i)$ for each agent $i$
        \STATE Take action $\bm{u}^t$, and retrieve next observation and reward $(\bm{o}^{t+1},r^t)$
        \STATE Store transition $(\bm{\tau}^t, \bm{u}^t, r^t, \bm{\tau}^{t+1})$ in $D$
        %\STATE $\bm{\tau}^{\text{temp}} = \bm{\tau'}$
        \STATE Sample a random minibatch of transitions $(\bm{\tau}, \bm{u}, r, \bm{\tau'})$ from $D$
         \STATE Set $y^{\text{dqn}}(r, \bm{\tau}'; \bm{\theta^{-}}) = r + \gamma
\Qtot(\bm{\tau}', \bm{\bar{u}}';\bm{\theta} ^{-}),$ $ \bar{\bm{u}}' = [\arg\max_{u_{i}}Q_i(\tau'_i,u_i;\bm{\theta}^{-})]_{i=1}^N,$
        \STATE update $\theta$ by minimizing the loss:
        \begin{align*}
L(\bm{\tau}, \bm{u}, r, \bm{\tau}'; \bm{\theta}) &=
 L_{\text{td}} + \lambda_{\text{opt}} L_{\text{opt}},\cr
L_{\text{td}}(\bm{\tau}, \bm{u}, r, \bm{\tau}';\bm{\theta}) &= \big(\Qtot(\bm{\tau},\bm{u}) - y^{\text{dqn}}(r, \bm{\tau}'; \bm{\theta}^{-})\big)^{2}.
        \end{align*}
        
        \begin{subequations}
  \begin{align*}[left ={L_{\text{opt}}(\bm{\tau}, \bm{u}, r, \bm{\tau}';\bm{\theta}) = \empheqlbrace}]
    & (\Qtot(\bm{\tau},\bm{u}) - \Qtot'(\bm{\tau},\bm{u}))^2         &\Qtot(\bm{\tau},\bm{u}) > \Qtot(\bm{\tau},\bm{\bar{u}}),  \\
    & (clip(\Qtot'(\bm{\tau},\bm{u}), \Qtot(\bm{\tau},\bm{\bar{u}}), \Qtot(\bm{\tau},\bm{u}))- \Qtot'(\bm{\tau},\bm{u}))^2  &\Qtot(\bm{\tau},\bm{u}) < \Qtot(\bm{\tau},\bm{\bar{u}}),
   \end{align*}
  \end{subequations}
  
        \STATE Update target network parameters $\theta^- = \theta$ with period $I$
        %\STATE $\bm{\tau} = \bm{\tau}^{\text{temp}}$
 \ENDFOR
 \ENDFOR
 \end{algorithmic}
 \end{algorithm}
 
%  \begin{subnumcases}{\hspace{-1.0cm}L_{\text{opt}}(;\bm{\theta})=}
%     \!\!\! (\Qtot(\bm{\tau},\bm{u}) - \Qtot'(\bm{\tau},\bm{u}))^2 & $\hspace{0.0cm}\Qtot(\bm{\tau},\bm{u}) > \Qtot(\bm{\tau},\bm{\bar{u}}),$ \\
%     \!\!\! (clip(\Qtot'(\bm{\tau},\bm{u}), \Qtot(\bm{\tau},\bm{\bar{u}}), \Qtot(\bm{\tau},\bm{u}))- \Qtot'(\bm{\tau},\bm{u}))^2 & $\hspace{0.0cm}\Qtot(\bm{\tau},\bm{u}) < \Qtot(\bm{\tau},\bm{\bar{u}}),$ \label{eq:regular_cond6}
% \end{subnumcases}


% can be readily factorized without changing the optimal actions in the original and the transformed joint action-value functions. 
%To this end, we jointly estimate $\Qtot$ and $\Qtot'$ as
% neural networks so as for $\Qtot'$ to be easily decomposed into
% individual action-value functions. 

% In Section~\ref{sec:transformation}, 
% if $\Qtot$ is factorizable, we study the conditions of $\Qtot$-factorizing $[Q_i]$ that is necessary and sufficient. Using this condition, in Section~\ref{sec:arch}, we propose a new deep RL framework $\algoname$ that aims at factorizing any factorizable joint action-value function $\Qtot.$  

% what condition $\Qtot$ is factorizable and prove that any factorizable
% action-value function is ensured to be factorized by this transform-based
% method. Next, we present the overall network architecture of
% $\algoname$, and elaborate on the details of its training and execution method. 






==> 5.relatedwork.tex <==
\section{Related Work}

Recently, several other methods have been proposed to solve the limitations of QMIX. \citet{mahajan2019maven} proposed MAVEN to address the issue with regards to exploration by using a committed exploration algorithm. \citet{yang2020multi} proposed Q-DPP which motivates agents to acquire diverse behavior models and to coordinate their exploration. However, they only experimented in a relatively simple environment like predator-prey. QPLEX \citep{wang2020qplex} takes a duplex dueling network architecture to factorize the joint value function. Unlike QTRAN, QPLEX learns using only one joint action-value network and a single loss function. Their experiments on the StarCraft Multi-Agent Challenge (SMAC) environment \citep{samvelyan19smac} also mainly utilized offline data. Finally, \citet{rashid2020weighted} proposed CW-QMIX and OW-QMIX which use a weighted projection that allows more emphasis to be placed on better joint actions. However, their methods are susceptible to weight parameter changes and the performance improvements have been demonstrated in limited SMAC environments only. Unlike these methods, we propose novel and simple-to-implement modifications that substantially improve the stability and performance of the original QTRAN.

